Automatic Diversity in the Software Supply Chain

Despite its obvious benefits, the increased adoption of package managers to automate the reuse of libraries has opened the door to a new class of hazards: supply chain attacks. By injecting malicious code in one library, an attacker may compromise all instances of all applications that depend on the library. To mitigate the impact of supply chain attacks, we propose the concept of Library Substitution Framework. This novel concept leverages one key observation: when an application depends on a library, it is very likely that there exists other libraries that provide similar features. The key objective of Library Substitution Framework is to enable the developers of an application to harness this diversity of libraries in their supply chain. The framework lets them generate a population of application variants, each depending on a different alternative library that provides similar functionalities. To investigate the relevance of this concept, we develop ARGO, a proof-of-concept implementation of this framework that harnesses the diversity of JSON suppliers. We study the feasibility of library substitution and its impact on a set of 368 clients. Our empirical results show that for 195 of the 368 java applications tested, we can substitute the original JSON library used by the client by at least 15 other JSON libraries without modifying the client's code. These results show the capacity of a Library Substitution Framework to diversify the supply chain of the client applications of the libraries it targets.

==> listings/Ill-formed.tex <==
\begin{lstlisting}[language=java, caption={Test excerpt from \jsonsimple checking forgiving behavior, removed from our curated test suite.}, label={lst:forgiving}]
s="[5,,2]";
obj=JSONValue.parse(s);
//ERROR_HANDLING
//assertEquals("[5,2]",obj.toString());
\end{lstlisting}

==> listings/jsonp-NAN.tex <==
\begin{lstlisting}[caption={Test excerpt from \gson testing serialization of Double\\ special values}, label={lst:jsonp-nan}]
JsonTreeWriter out = new JsonTreeWriter();
out.setLenient(true);
out.beginArray();
out.value(Double.NaN);
out.value(Double.NEGATIVE_INFINITY);
out.value(Double.POSITIVE_INFINITY);
out.endArray();
assertEquals("[NaN,-Infinity,Infinity]",
        out.get().toString());
\end{lstlisting}

==> listings/jsonutil-key.tex <==
\begin{lstlisting}[caption={Test excerpt from \jsonsimple testing serialization\\ and deserialization of arrays and objects}, label={lst:jsonutil-key}]
String s = "[0,{\"1\":{\"2\":{\"3\":"
   + "{\"4\":[5,{\"6\":7}]}}}}]";
Object obj = JSONValue.parse(s);
JSONArray array = (JSONArray) obj;
assertEquivalent("{\"1\":{\"2\":{\"3\":"
   + "{\"4\":[5,{\"6\":7}]}}}}",
   array.get(1).toString());
\end{lstlisting}


==> listings/mjson-unsupported.tex <==
\begin{lstlisting}[language=java, caption={Test excerpt from \jsonsimple removing an entry\\ in a \json object}, label={lst:remove}]
JSONObject obj1= new JSONObject();
obj1.remove("array1");
\end{lstlisting}

==> listings/over-assumption.tex <==
\begin{lstlisting}[language=java, caption={Test excerpt from vertx-maven-plugin  ConfigConversionUtilTest\#convertSimpleYamlToJson}, label={lst:long-int}]
        //{"http.port":8080}
        JSONObject jsonMap = new JSONObject(jsonDoc);
        assertNotNull(jsonMap);
        assertEquals(8080, jsonMap.get("http.port"));
        //expected: java.lang.Integer<8080> but was: java.lang.Long<8080>
\end{lstlisting}

%org.json to json-simple/gson

%https://github.com/reactiverse/vertx-maven-plugin/blob/5210e55e4cfbac4e134f3344eb81cfcb7b00bac8/src/test/java/io/reactiverse/vertx/maven/plugin/ConfigConversionUtilTest.java#L47

%Note that JSONObject has a method Integer getInteger(String)

==> listings/pom-diff.tex <==
\begin{lstlisting}[language=diff, caption={Excerpt of \texttt{jitsi-videobridge}'s pom.xml diff illustrating\\ a change from \texttt{json-simple} to \texttt{json}}, label={lst:pom-diff}]
- <dependency>
-   <groupId>com.googlecode.json-simple</groupId>
-   <artifactId>json-simple</artifactId>
-   <version>1.1.1</version>
- </dependency>
+ <dependency>
+   <groupId>se.kth.castor</groupId>
+   <artifactId>json-over-argo</artifactId>
+   <version>1.0-SNAPSHOT</version>
+ </dependency>
+ <dependency>
+   <groupId>se.kth.castor</groupId>
+   <artifactId>argo-json</artifactId>
+   <version>1.0-SNAPSHOT</version>
+ </dependency>
\end{lstlisting}

==> listings/unicode.tex <==
\begin{CJK}{UTF8}{}
\begin{Japanese}
\begin{lstlisting}[caption={Test excerpt from \jsonsimple testing support for\\ unicode characters}, label={lst:unicode},extendedchars=false]
String s = "[\"hello\\bworld\\\"abc\\tdef"
   + "\\\\ghi\\rjkl\\n123\ \u4e2d\"]";
Object obj = JSONValue.parse(s);
assertEquals("hello\bworld\"abc\tdef"
   + "\\ghi\rjkl\n123 中",
   ((List)obj).get(0).toString());
\end{lstlisting}
\end{Japanese}
\end{CJK}

==> listings/unsupported.tex <==
\begin{lstlisting}[language=java, caption={Test excerpt from \json checking an error message}, label={lst:error-handling}]
try {
    jsonObject.getBoolean("stringKey");
    fail("Expected an exception");
} catch (JSONException e) {
    assertEquals("Expecting an exception message", 
            "JSONObject[\"stringKey\"] is not a Boolean.",
            e.getMessage());
}
\end{lstlisting}

==> tables/api.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}llrrr@{}}
  \toprule
  \textsc{Library} & \textsc{API} & \textsc{Full} & \textsc{Used} & \textsc{Tradeoff} \\ 
  \midrule
   & Package &   8 &   8 &   6 \\ 
  gson & Type &  65 & 294 &  32 \\ 
   & Element & 517 & 1972 & 205 \\  
  \midrule
   & Package &  20 &  19 &  13 \\ 
  jackson & Type & 519 & 298 &  62 \\ 
   & Element & 7954 & 2254 & 340 \\ 
  \midrule 
   & Package &   2 &   2 &   2 \\ 
  json-simple & Type &  11 &  15 &   9 \\ 
   & Element & 102 & 162 &  70 \\ 
  \midrule 
   & Package &   1 &   1 &   1 \\ 
  json & Type &  19 &  32 &  14 \\ 
   & Element & 248 & 423 & 208 \\  
  \midrule
   & Package &  15 &  15 &   7 \\ 
  fastjson & Type & 168 & 228 &  24 \\ 
   & Element & 1959 & 2474 & 158 \\ 
  \bottomrule
\end{tabular}
\end{table}

==> tables/compilation.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lrr}
  \hline
 \textsc{Bridge}  & \textsc{\# Clients} & \textsc{\#Compile} \\ 
  \hline
 jackson-databind & 128 & 115 (89.84\%) \\
 gson & 122 & 117 (95.90\%)  \\ 
 json-simple &  34 &  29 (85.29\%) \\ 
 json &  84  &  68 (80.95\%)\\ 
   \hline
 Total &  368 &  329 (89.40\%) \\ 
   \hline
\end{tabular}
\vspace{0.5em}
\caption{Compilation outcome of clients after replacement of the \json library by its corresponding bridge.}
\label{tab:compilation}
\end{table}

==> tables/cross_tests_results_old.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lrrrr}
  \hline
\textsc{Implementation} & \textsc{gson} & \textsc{jackson} & \textsc{json} & \textsc{json-simple} \\ 
  \hline
  cookjson & \cellcolor{green!25}0/133 & \cellcolor{yellow!25}6/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  corn & \cellcolor{green!25}0/133 & \cellcolor{yellow!25}5/141 & \cellcolor{yellow!25}6/89 & \cellcolor{green!25}0/27 \\ 
  fastjson & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  flexjson & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}1/89 & \cellcolor{green!25}0/27 \\ 
  genson & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  gson & \cellcolor{green!25}0/133 & \cellcolor{yellow!25}4/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  jackson-databind & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}3/89 & \cellcolor{green!25}0/27 \\ 
  jjson & \cellcolor{yellow!25}2/133 & \cellcolor{yellow!25}10/141 & \cellcolor{red!25}18/89 & \cellcolor{yellow!25}2/27 \\ 
  johnzon & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{yellow!25}1/27 \\ 
  json & \cellcolor{yellow!25}1/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  json-argo & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}1/89 & \cellcolor{yellow!25}1/27 \\ 
  json-io & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}1/89 & \cellcolor{green!25}0/27 \\ 
  json-lib & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  json-simple & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}1/89 & \cellcolor{green!25}0/27 \\ 
  jsonij & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  jsonp & \cellcolor{yellow!25}1/133 & \cellcolor{yellow!25}7/141 & \cellcolor{green!25}0/89 & \cellcolor{green!25}0/27 \\ 
  jsonutil & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}1/89 & \cellcolor{yellow!25}1/27 \\ 
  mjson & \cellcolor{red!25}20/133 & \cellcolor{red!25}22/141 & \cellcolor{red!25}26/89 & \cellcolor{yellow!25}2/27 \\ 
  progbase-json & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{red!25}10/89 & \cellcolor{green!25}0/27 \\ 
  sojo & \cellcolor{green!25}0/133 & \cellcolor{green!25}0/141 & \cellcolor{yellow!25}2/89 & \cellcolor{yellow!25}2/27 \\ 
   \hline
  Total successes & 16/20 & 14/20 & 9/20 & 14/20 \\ 
   \hline
\end{tabular}
\vspace{0.5em}
\caption{Failure matrix for test for the \nbsrcjson bridges on the \nbtargetjson implementations}
\label{tab:cross-test-results}
\end{table}

==> tables/libraries.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lrrrr@{}}
  \toprule
\textsc{Library} & \textsc{\# Commits} & \textsc{\# Stars} & \textsc{Version} & \textsc{Last activity} \\ 
  \midrule
  cookjson & 116 & 3 & 1.0.2 & Sept 2017 \\ 
  corn & - & - & 1.0.8 & Feb 14 \\ 
  fastjson & 3793 & 1.4k & 1.2.75 & Nov 2020 \\ 
  flexjson & - & - & 3.3 & Oct 2014 \\ 
  genson & 395 & 193 & 1.6 & Dec 2019 \\ 
  gson & 1485 & 18.8k & 2.8.5 & May 2020 \\ 
  jackson & 7382 & 2.7k & 2.12.0-rc2 & Nov 2020 \\ 
  jjson & 216 & 12 & 0.1.7 & Jul 2016 \\ 
  johnzon & 780 & - & 1.1.8 & Nov 2020 \\ 
  json & 841 & 3.7k & 20201115 & Nov 2020 \\ 
  json-argo & - & - & 5.13 & Nov 2020 \\ 
  json-io & 1040 & 268 & 4.12.0 & Oct 2013 \\ 
  json-lib & - & - & 3.0.1 & Dec 2010 \\ 
  json-simple & - & 594 & 1.1.1 & Jul 2014 \\ 
  json-util & 464 & 48 & 1.10.4-java7 & Oct 16 \\ 
  jsonij & 348 & - & 0.3.1 & Feb 2020 \\ 
  jsonp & 530 & 75 & 2.0.0 & Nov 18 \\ 
  mjson & 79 & 67 & 1.4.0 & May 19 \\ 
  progbase & - & - & 0.4.0 & Nov 2019 \\ 
  sojo & - & - & 1.0.13 & Feb 2019 \\ 
   \bottomrule 
\end{tabular}
    \vspace{0.5em}
    \caption{Description of the \json libraries studied by \textit{Harrand et al.}~\cite{harrandjson}}
    \label{tab:libs}
\end{table}

==> tables/libraries_new.tex <==
\begin{table}[ht]
\centering
\rowcolors{2}{gray!25}{white}
\begin{tabular}{@{}lrrrrrr@{}}
  %\toprule
%\textsc{Library} & \rotatebox{90}{\textsc{\#Version}} & \rotatebox{90}{\textsc{\#API\_Elements}} & \rotatebox{90}{\textsc{Chosen\_Version}} \\ 
%\textsc{Library} & 
%\rotatebox{90}{\textsc{\#Versions}} & 
%\rotatebox{90}{\textsc{\#API\_Elements}} & 
%\rotatebox{90}{\textsc{Chosen\_Version}} & 
%\rotatebox{90}{\textsc{Bridged}} \\ 
\textsc{Library} & 
\textsc{\#Versions} & 
\textsc{API Size} & 
\textsc{Version} & 
\textsc{Bridged} \\ 
  \midrule
jackson & 159 & 5807 & 2.12.0-rc2 & \checkmark  \\
gson & 31 & 468 & 2.8.5 & \checkmark  \\
json & 19 & 301 & 20201115 & \checkmark  \\
json-simple & 2 & 102 & 1.1.1 & \checkmark  \\
  \midrule
fastjson & 221 & 1860 & 1.2.75 &  \\
sojo & 3 & 788 & 1.0.13 &  \\
genson & 21 & 747 & 1.6 &  \\
json-lib & 14 & 651 & 3.0.1 &  \\
jsonij & 12 & 714 & 0.3.1 &  \\
jsonp & 7 & 392 & 2.0.0 &  \\
flexjson & 6 & 326 & 3.3 &  \\
progbase & 3 & 312 & 0.4.0 &  \\
json-util & 77 & 296 & 1.10.4-java7 &  \\
cookjson & 3 & 279 & 1.0.2 &  \\
json-io & 11 & 230 & 4.12.0 &  \\
json-argo & 68 & 221 & 5.13 &  \\
johnzon & 44 & 199 & 1.1.8 &  \\
corn & 9 & 146 & 1.0.8 &  \\
mjson & 5 & 77 & 1.4.0 &  \\
jjson & 3 & 42 & 0.1.7 &  \\
   \bottomrule 
\end{tabular}
    \vspace{0.5em}
    \caption{Description of the \json reservoir\\ We reuse the 20 \json libraries studied in previous work~\cite{harrandjson}.}
    \label{tab:libs-api}
\end{table}

==> tables/library_apis.tex <==
\begin{table}[ht]
\centering
\rowcolors{2}{gray!25}{white}
\begin{tabular}{@{}lrrrrrrr@{}}
  %\toprule
\textsc{Library} & \rotatebox{90}{\textsc{\#Version}} & \rotatebox{90}{\textsc{\#API\_Elements}} & \rotatebox{90}{\textsc{\#API\_Bridge}} & \rotatebox{90}{\textsc{\#API\_Wrapper}} & \rotatebox{90}{\textsc{Chosen\_Version}} \\ 
  \midrule
jackson-databind & 159 & 5807 & 79 & 36 & 2.12.0-rc2  \\
fastjson & 221 & 1860 & - & 12 & 1.2.75  \\
sojo & 3 & 788 & - & 4 & 1.0.13  \\
genson & 21 & 747 & - & 4 & 1.6  \\
json-lib & 14 & 651 & - & 5 & 3.0.1  \\
jsonij & 12 & 714 & - & 11 & 0.3.1  \\
gson & 31 & 468 & 60 & 26 & 2.8.5  \\
jsonp & 7 & 392 & - & 14 & 2.0.0  \\
flexjson & 6 & 326 & - & 6 & 3.3  \\
progbase & 3 & 312 & - & 2 & 0.4.0  \\
json & 19 & 301 & 123 & 9 & 20201115  \\
json-util & 77 & 296 & - & 2 & 1.10.4-java7  \\
cookjson & 3 & 279 & - & 23 & 1.0.2  \\
json-io & 11 & 230 & - & 6 & 4.12.0  \\
json-argo & 68 & 221 & - & 34 & 5.13  \\
johnzon & 44 & 199 & - & 13 & 1.1.8  \\
corn & 9 & 146 & - & 21 & 1.0.8  \\
json-simple & 2 & 102 & 74 & 8 & 1.1.1  \\
mjson & 5 & 77 & - & 71 & 1.4.0  \\
jjson & 3 & 42 & - & 19 & 0.1.7  \\
   \bottomrule 
\end{tabular}
    \vspace{0.5em}
    \caption{Description of the APIs of the \json reservoir}
    \label{tab:libs-api}
\end{table}

==> tables/supported_assertions.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{@{}lrrrrrr|rr@{}}
  \textsc{Library} & \rotatebox{90}{\textsc{ORIGINAL}} & \rotatebox{90}{\textsc{EQUIVALENT}} & \rotatebox{90}{\textsc{PLACEBO}} & \rotatebox{90}{\textsc{FEAT\_IGNORED}} & \rotatebox{90}{\textsc{ERROR\_HANDLING}} & \rotatebox{90}{\textsc{MISC.}} &  \rotatebox{90}{\textsc{TOTAL\_KEPT}} &  \rotatebox{90}{\textsc{TESTS\_KEPT}} \\ 
  \midrule
  gson & 355 & 7 & 1853 & 0 & 2 & 0 & 362 & 133 / 1051\\ 
  jackson & 795 & 94 & 7821 & 0 & 3 & 8 & 889 & 141 / 2473\\ 
  json & 400 & 42 & 18 & 539 & 82 & 16 & 442 & 84 / 93\\ 
  json-simple & 44 & 128 & 0 & 19 & 6 & 0 & 172 & 27 / 28 \\ 
  \bottomrule
\end{tabular}
\vspace{1em}
\caption{Cross library testing overview}
\label{tab:assert}
\end{table}

%Original
%intention

==> tables/test_outcome.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{r|rrrrr|r}
 \textsc{Bridge} & \rotatebox{90}{\textsc{\#CLIENTS}} & \rotatebox{90}{\textsc{\#NO\_ALTERNATIVES}} & \rotatebox{90}{\textsc{\#SOME\_ALTERNATIVES}} & \rotatebox{90}{\textsc{\#20\_ALTERNATIVES}} & \rotatebox{90}{\textsc{\#ACCEPTABLE}} &  \rotatebox{90}{\textsc{\#TOTAL\_ALTERNATIVES}} \\ 
  \midrule
  gson & 117 &  12 &  66 &  39 & 105 (90\%) & 1,576 \\ 
  jackson-databind & 115 &  27 &  49 &  39 &  88 (77\%) & 1,469 \\ 
  json &  68 &  13 &  48 &   7 &  55 (81\%) & 754 \\ 
  json-simple &  29 &   5 &  21 &   3 &  24 (83\%) & 270 \\ 
  \midrule
  Total & 329 &  57 & 184 &  88 & 272 (83\%) & 4,069 \\ 
   \bottomrule 
\end{tabular}
\vspace{1em}
\caption{Overview of client alternative \json suppliers provided by \argo}
\label{tab:test-outcome}
\end{table}
